Formalizing Constructive Quantifier Elimination in Agda

In this paper a constructive formalization of quantifier elimination is presented, based on a classical formalization by Tobias Nipkow. The formalization is implemented and verified in the programming language/proof assistant Agda. It is shown that, as in the classical case, the ability to eliminate a single existential quantifier may be generalized to full quantifier elimination and consequently a decision procedure. The latter is shown to have strong properties under a constructive metatheory, such as the generation of witnesses and counterexamples. Finally, this is demonstrated on a minimal theory on the natural numbers.

==> eptcsdata.tex <==
\providecommand{\firstpage}{2}
\providecommand{\publicationstatus}{R. Atkey and S. Lindley (Eds.): Mathematically\\
Structured Functional Programming (MSFP 2018)\\
EPTCS 275, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.275.2}{10.4204/EPTCS.275.2}}

